Generative Well-intentioned Networks

We propose Generative Well-intentioned Networks (GWINs), a novel framework for increasing the accuracy of certainty-based, closed-world classifiers. A conditional generative network recovers the distribution of observations that the classifier labels correctly with high certainty. We introduce a reject option to the classifier during inference, allowing the classifier to reject an observation instance rather than predict an uncertain label. These rejected observations are translated by the generative network to high-certainty representations, which are then relabeled by the classifier. This architecture allows for any certainty-based classifier or rejection function and is not limited to multilayer perceptrons. The capability of this framework is assessed using benchmark classification datasets and shows that GWINs significantly improve the accuracy of uncertain observations.

==> __latexindent_temp.tex <==
@article{ghahramani2015probabilistic,
  title={Probabilistic machine learning and artificial intelligence},
  author={Ghahramani, Zoubin},
  journal={Nature},
  volume={521},
  number={7553},
  pages={452},
  year={2015},
  publisher={Nature Publishing Group}
}

@phdthesis{gal2016uncertainty,
  title={Uncertainty in Deep Learning},
  author={Gal, Yarin},
  year={2016},
  school={University of Cambridge}
}

@inproceedings{kingma2015variational,
  title={Variational dropout and the local reparameterization trick},
  author={Kingma, Durk P and Salimans, Tim and Welling, Max},
  booktitle={Advances in Neural Information Processing Systems},
  pages={2575--2583},
  year={2015}
}


@misc{gal2015bayesian,
    title={Bayesian Convolutional Neural Networks with Bernoulli Approximate Variational Inference},
    author={Yarin Gal and Zoubin Ghahramani},
    year={2015},
    eprint={1506.02158},
    archivePrefix={arXiv},
    primaryClass={stat.ML}
}

@inproceedings{gal2016dropout,
  title={Dropout as a bayesian approximation: Representing model uncertainty in deep learning},
  author={Gal, Yarin and Ghahramani, Zoubin},
  booktitle={International Conference on Machine Learning},
  pages={1050--1059},
  year={2016}
}

@inproceedings{gal2016theoretically,
  title={A theoretically grounded application of dropout in recurrent neural networks},
  author={Gal, Yarin and Ghahramani, Zoubin},
  booktitle={Advances in Neural Information Processing Systems},
  pages={1019--1027},
  year={2016}
}

@article{mackay1992practical,
  title={A practical Bayesian framework for backpropagation networks},
  author={MacKay, David JC},
  journal={Neural computation},
  volume={4},
  number={3},
  pages={448--472},
  year={1992},
  publisher={MIT Press}
}

@phdthesis{neal2012bayesian,
  title={Bayesian learning for neural networks},
  author={Neal, Radford M},
  year={1995},
  school={University of Toronto}
}

@article{chow1970optimum,
  title={On optimum recognition error and reject tradeoff},
  author={Chow, Chi-Keung},
  journal={IEEE Transactions on information theory},
  volume={16},
  number={1},
  pages={41--46},
  year={1970},
  publisher={IEEE}
}

@inproceedings{goodfellow2014generative,
  title={Generative adversarial nets},
  author={Goodfellow, Ian and Pouget-Abadie, Jean and Mirza, Mehdi and Xu, Bing and Warde-Farley, David and Ozair, Sherjil and Courville, Aaron and Bengio, Yoshua},
  booktitle={Advances in Neural Information Processing Systems},
  pages={2672--2680},
  year={2014}
}

@inproceedings{salimans2016improved,
  title={Improved techniques for training gans},
  author={Salimans, Tim and Goodfellow, Ian and Zaremba, Wojciech and Cheung, Vicki and Radford, Alec and Chen, Xi},
  booktitle={Advances in Neural Information Processing Systems},
  pages={2234--2242},
  year={2016}
}

@inproceedings{
  wang2018function,
  title={Function Space Particle Optimization for Bayesian Neural Networks},
  author={Ziyu Wang and Tongzheng Ren and Jun Zhu and Bo Zhang},
  booktitle={International Conference on Learning Representations},
  year={2019},
  url={https://openreview.net/forum?id=BkgtDsCcKQ},
}

@InProceedings{shi2018spectral,
  title = 	 {A Spectral Approach to Gradient Estimation for Implicit Distributions},
  author = 	 {Shi, Jiaxin and Sun, Shengyang and Zhu, Jun},
  booktitle = 	 {Proceedings of the 35th International Conference on Machine Learning},
  pages = 	 {4651--4660},
  year = 	 {2018},
}

@misc{shi2017zhusuan,
    title={ZhuSuan: A Library for Bayesian Deep Learning},
    author={Jiaxin Shi and Jianfei Chen and Jun Zhu and Shengyang Sun and Yucen Luo and Yihong Gu and Yuhao Zhou},
    year={2017},
    eprint={1709.05870},
    archivePrefix={arXiv},
    primaryClass={stat.ML}
}

@misc{arjovsky2017wasserstein,
  title={Wasserstein GAN},
  author={Martin Arjovsky and Soumith Chintala and Léon Bottou},
  year={2017},
  eprint={1701.07875},
  archivePrefix={arXiv},
  primaryClass={stat.ML}
}

@inproceedings{gulrajani2017improved,
  title={Improved training of wasserstein gans},
  author={Gulrajani, Ishaan and Ahmed, Faruk and Arjovsky, Martin and Dumoulin, Vincent and Courville, Aaron C},
  booktitle={Advances in Neural Information Processing Systems},
  pages={5767--5777},
  year={2017}
}

@misc{mirza2014conditional,
    title={Conditional Generative Adversarial Nets},
    author={Mehdi Mirza and Simon Osindero},
    year={2014},
    eprint={1411.1784},
    archivePrefix={arXiv},
    primaryClass={cs.LG}
}

@article{chow1957optimum,
  title={An optimum character recognition system using decision functions},
  author={Chow, Chi-Keung},
  journal={IRE Transactions on Electronic Computers},
  number={4},
  pages={247--254},
  year={1957},
  publisher={IEEE}
}

@inproceedings{tortorella2000optimal,
  title={An optimal reject rule for binary classifiers},
  author={Tortorella, Francesco},
  booktitle={Joint IAPR International Workshops on Statistical Techniques in Pattern Recognition (SPR) and Structural and Syntactic Pattern Recognition (SSPR)},
  pages={611--620},
  year={2000},
  organization={Springer}
}

@article{bartlett2008classification,
  title={Classification with a reject option using a hinge loss},
  author={Bartlett, Peter and Wegkamp, Marten},
  journal={Journal of Machine Learning Research},
  volume={9},
  number={8},
  pages={1823--1840},
  year={2008}
}

@inproceedings{cortes2016learning,
  title={Learning with rejection},
  author={Cortes, Corinna and DeSalvo, Giulia and Mohri, Mehryar},
  booktitle={International Conference on Algorithmic Learning Theory},
  pages={67--82},
  year={2016},
  organization={Springer}
}

@article{lecun1998gradient,
  title={Gradient-based learning applied to document recognition},
  author={LeCun, Yann and Bottou, L{\'e}on and Bengio, Yoshua and Haffner, Patrick},
  journal={Proceedings of the IEEE},
  volume={86},
  number={11},
  pages={2278--2324},
  year={1998},
  publisher={IEEE}
}

@misc{dillon2017tensorflow,
  title={TensorFlow Distributions},
  author={Joshua V. Dillon and Ian Langmore and Dustin Tran and Eugene Brevdo and Srinivas Vasudevan and Dave Moore and Brian Patton and Alex Alemi and Matt Hoffman and Rif A. Saurous},
  year={2017},
  eprint={1711.10604},
  archivePrefix={arXiv},
  primaryClass={cs.LG}
}

@inproceedings{wen2018flipout,
  title={Flipout: Efficient Pseudo-Independent Weight Perturbations on Mini-Batches},
  author={Yeming Wen and Paul Vicol and Jimmy Ba and Dustin Tran and Roger Grosse},
  booktitle={International Conference on Learning Representations},
  year={2018},
  url={https://openreview.net/forum?id=rJNpifWAb},
}

@misc{xiao2017fashion,
    title={Fashion-MNIST: a Novel Image Dataset for Benchmarking Machine Learning Algorithms},
    author={Han Xiao and Kashif Rasul and Roland Vollgraf},
    year={2017},
    eprint={1708.07747},
    archivePrefix={arXiv},
    primaryClass={cs.LG}
}

@inproceedings{donahue2016adversarial,
  title={Adversarial Feature Learning},
  author={Donahue, Jeff and Kr{\"a}henb{\"u}hl, Philipp and Darrell, Trevor},
  booktitle={International Conference on Learning Representations},
  year={2017}
}

@inproceedings{dumoulin2016adversarially,
  title={Adversarially learned inference},
  author={Dumoulin, Vincent and Belghazi, Ishmael and Poole, Ben and Mastropietro, Olivier and Lamb, Alex and Arjovsky, Martin and Courville, Aaron},
  booktitle={International Conference on Learning Representations},
  year={2017}
}

@inproceedings{chongxuan2017triple,
  title={Triple generative adversarial nets},
  author={Li, Chongxuan and Xu, Taufik and Zhu, Jun and Zhang, Bo},
  booktitle={Advances in Neural Information Processing Systems},
  pages={4088--4098},
  year={2017}
}

@inproceedings{samangouei2018defense,
  title={Defense-GAN: Protecting classifiers against adversarial attacks using generative models},
  author={Samangouei, Pouya and Kabkab, Maya and Chellappa, Rama},
  booktitle={International Conference on Learning Representations},
  year={2018}
}

@inproceedings{reed2016generative,
  author={Scott Reed and Zeynep Akata and Xinchen Yan and Lajanugen Logeswaran and Bernt Schiele and Honglak Lee},
  title={Generative Adversarial Text to Image Synthesis},
  booktitle = {Proceedings of the 33rd International Conference on International Conference on Machine Learning - Volume 48},
  series = {ICML'16},
  year = {2016},
  location = {New York, NY, USA},
  pages = {1060--1069},
  numpages = {10},
  url = {http://dl.acm.org/citation.cfm?id=3045390.3045503},
  acmid = {3045503},
  publisher = {JMLR.org},
}

@inproceedings{miyato2018cgans,
  title={c{GAN}s with Projection Discriminator},
  author={Takeru Miyato and Masanori Koyama},
  booktitle={International Conference on Learning Representations},
  year={2018},
  url={https://openreview.net/forum?id=ByS1VpgRZ},
}

@inproceedings{odena2017conditional,
  title={Conditional image synthesis with auxiliary classifier gans},
  author={Odena, Augustus and Olah, Christopher and Shlens, Jonathon},
  booktitle={Proceedings of the 34th International Conference on Machine Learning-Volume 70},
  pages={2642--2651},
  year={2017},
  organization={JMLR. org}
}

@inproceedings{zhang2017stackgan,
  title={Stackgan: Text to photo-realistic image synthesis with stacked generative adversarial networks},
  author={Zhang, Han and Xu, Tao and Li, Hongsheng and Zhang, Shaoting and Wang, Xiaogang and Huang, Xiaolei and Metaxas, Dimitris N},
  booktitle={Proceedings of the IEEE International Conference on Computer Vision},
  pages={5907--5915},
  year={2017}
}

@inproceedings{lakshminarayanan2017simple,
  title={Simple and scalable predictive uncertainty estimation using deep ensembles},
  author={Lakshminarayanan, Balaji and Pritzel, Alexander and Blundell, Charles},
  booktitle={Advances in Neural Information Processing Systems},
  pages={6402--6413},
  year={2017}
}

@inproceedings{geifman2019selectivenet,
  title = 	 {{S}elective{N}et: A Deep Neural Network with an Integrated Reject Option},
  author = 	 {Geifman, Yonatan and El-Yaniv, Ran},
  booktitle = 	 {Proceedings of the 36th International Conference on Machine Learning},
  pages = 	 {2151--2159},
  year = 	 {2019},
  editor = 	 {Chaudhuri, Kamalika and Salakhutdinov, Ruslan},
  volume = 	 {97},
  series = 	 {Proceedings of Machine Learning Research},
  address = 	 {Long Beach, California, USA},
  month = 	 {09--15 Jun},
  publisher = 	 {PMLR},
  pdf = 	 {http://proceedings.mlr.press/v97/geifman19a/geifman19a.pdf},
  url = 	 {http://proceedings.mlr.press/v97/geifman19a.html},
}

@inproceedings{geifman2019selective,
 author = {Geifman, Yonatan and El-Yaniv, Ran},
 title = {Selective Classification for Deep Neural Networks},
 booktitle = {Proceedings of the 31st International Conference on Neural Information Processing Systems},
 series = {NIPS'17},
 year = {2017},
 isbn = {978-1-5108-6096-4},
 location = {Long Beach, California, USA},
 pages = {4885--4894},
 numpages = {10},
 url = {http://dl.acm.org/citation.cfm?id=3295222.3295241},
 acmid = {3295241},
 address = {USA},
}

@inproceedings{meng2017magnet,
 author = {Meng, Dongyu and Chen, Hao},
 title = {MagNet: A Two-Pronged Defense Against Adversarial Examples},
 booktitle = {Proceedings of the 2017 ACM SIGSAC Conference on Computer and Communications Security},
 series = {CCS '17},
 year = {2017},
 isbn = {978-1-4503-4946-8},
 location = {Dallas, Texas, USA},
 pages = {135--147},
 numpages = {13},
 url = {http://doi.acm.org/10.1145/3133956.3134057},
 doi = {10.1145/3133956.3134057},
 acmid = {3134057},
 address = {New York, NY, USA},
 keywords = {adversarial example, autoencoder, neural network},
}

@inproceedings{papernot2016distillation,
  title={Distillation as a defense to adversarial perturbations against deep neural networks},
  author={Papernot, Nicolas and McDaniel, Patrick and Wu, Xi and Jha, Somesh and Swami, Ananthram},
  booktitle={2016 IEEE Symposium on Security and Privacy (SP)},
  pages={582--597},
  year={2016},
  organization={IEEE}
}

@misc{goodfellow2014explaining,
    title={Explaining and Harnessing Adversarial Examples},
    author={Ian J. Goodfellow and Jonathon Shlens and Christian Szegedy},
    year={2014},
    eprint={1412.6572},
    archivePrefix={arXiv},
    primaryClass={stat.ML}
}

@misc{antoniou2017data,
    title={Data Augmentation Generative Adversarial Networks},
    author={Antreas Antoniou and Amos Storkey and Harrison Edwards},
    year={2017},
    eprint={1711.04340},
    archivePrefix={arXiv},
    primaryClass={stat.ML}
}

@inproceedings{hariharan2017low,
  title={Low-shot visual recognition by shrinking and hallucinating features},
  author={Hariharan, Bharath and Girshick, Ross},
  booktitle={Proceedings of the IEEE International Conference on Computer Vision},
  pages={3018--3027},
  year={2017}
}

@inproceedings{wang2018low,
  title={Low-shot learning from imaginary data},
  author={Wang, Yu-Xiong and Girshick, Ross and Hebert, Martial and Hariharan, Bharath},
  booktitle={Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition},
  pages={7278--7286},
  year={2018}
}

